Multilingual Generative Language Models for Zero-Shot Cross-Lingual Event Argument Extraction

We present a study on leveraging multilingual pre-trained generative language models for zero-shot cross-lingual event argument extraction (EAE). By formulating EAE as a language generation task, our method effectively encodes event structures and captures the dependencies between arguments. We design language-agnostic templates to represent the event argument structures, which are compatible with any language, hence facilitating the cross-lingual transfer. Our proposed model finetunes multilingual pre-trained generative language models to generate sentences that fill in the language-agnostic template with arguments extracted from the input passage. The model is trained on source languages and is then directly applied to target languages for event argument extraction. Experiments demonstrate that the proposed model outperforms the current state-of-the-art models on zero-shot cross-lingual EAE. Comprehensive studies and error analyses are presented to better understand the advantages and the current limitations of using generative language models for zero-shot cross-lingual transfer EAE.

==> 99-error-analysis.tex <==
\section{Error Categories}
\label{app:detail_err}
In Section~\ref{subsec:err}, we present error analysis on \model{} (mT5-base). In this section, we detail the categories that we used for that study.



\paragraph{Errors on both monolingual and cross-lingual model.} We compare the predicted results from \model{}(ar $\Rightarrow$ en) with \model{}(en $\Rightarrow$ en), or from \model{}(zh $\Rightarrow$ en) with \model{}(en $\Rightarrow$ en).
If their predictions are similar and both of them are wrong when compared to the gold output, we classify the error to this category. To overcome the errors in this category, the potential solution is to improve monolingual models for EAE tasks.

\paragraph{Over generate.} 
Errors in this category happen more often in \model{}(ar $\Rightarrow$ en). It is likely because the entities in Arabic are usually much longer than that in English, when measuring by the number of sub-words. Based on our statistics, the average entity span length is 2.85 for Arabic, and is 2.00 for English (length of sub-words). This leads to the natural for our \model{}(ar $\Rightarrow$ en) to overly generate some tokens even though they have captured the correct concept.
An example is that the model predicts \textit{``The EU foreign ministers''}, while the ground truth is \textit{``ministers''}.

\paragraph{Label disagreement on different language split.}
The annotations for the ACE dataset in different language split contain some ambiguity. For example, given sentence \textit{``He now also advocates letting in U.S. troops for a war against Iraq even though it is a fellow Muslim state.''} and the queried trigger \textit{``war''}, the annotations in English tends to label \textit{Iraq} as the \textit{Place} where the event happen, while similar situations in other languages will mark \textit{Iraq} as the \textit{Target} for the war.

\paragraph{Grammar difference between languages.}
An example for this category is \textit{``... Blackstone Group would buy Vivendi's theme park division, including Universal Studios Hollywood ...''} and the queried trigger \textit{``buy''}. 
We observe that \model{}(ar $\Rightarrow$ en) predicts \textit{Videndi} as the \textit{Artifact} been sold and \textit{division} is the \textit{Seller}, while \model{}(en $\Rightarrow$ en) can correctly understand that \textit{Videndi} are the \textit{Seller} and \textit{division} is the \textit{Artifact}. 
We hypothesize the reason being the differences between the grammar in Arabic and English.
The word order of the sentence \textit{``Vivendi's theme park division''} in Arabic is reversed with its English counterpart, that is, \textit{``theme park division''} will be written before \textit{``Vivendi''} in Arabic. Such difference leads to the errors in this category.


\paragraph{Generate a word that is not in the passage.}

In \model{}(zh $\Rightarrow$ en), we observe several errors regarding generating a word that is not in the passage. There are two typical situations. The first case is that \model{}(zh $\Rightarrow$ en) presents difficulty understanding singular and plural nouns. For example, the model will generate \textit{``studios''} as prediction while only \textit{``studio''} appear in the passage. This is because the concept regarding the differences between singular and plural nouns are less emphasized in Chinese. The second cases is that \model{}(zh $\Rightarrow$ en) will generate random predictions in Chinese.

\paragraph{Generate a correct prediction, but in Chinese.}
This is a special case of \textit{``Generate a word that is not in the passage''}. In this category, we observe that although the prediction is in Chinese (hence, a wrong prediction), it is correct if we translate the prediction into English. 


From these examples, we highlight two remaining challenges for future studies. First, there are several errors raising because of the discrepancies between the source language and the target language, such as the output length distribution mismatching or the grammar differences. 
Prior works like GATE~\cite{Wasi21gate} use pos-tags and dependency parsing to mitigate the grammar difference, and we leave it as a future work to study how to leverage such supplementary information into the generation-based framework. Also, a potential research question on how to alleviate the language differences in zero-shot cross-lingual transfer tasks.

Second, we demonstrate that even though we have already incorporated copy mechanism to facilitate the generation in target language, it is still challenging for the model to be fully controlled when adapting to cross-lingual cases. In Section~\ref{subsec:err}, we have already presented the results of applying constrained decoding to alleviate such errors. However, the improvement on cross-lingual transfer cases sacrifice the monolingual results. This raise a future research question --- whether we can control the generation more ``softly'' so that the improvement can be consistent on both monolingual cases and cross-lingual cases.
